Eyes are the Windows to the Soul: Predicting the Rating of Text Quality Using Gaze Behaviour

Predicting a reader's rating of text quality is a challenging task that involves estimating different subjective aspects of the text, like structure, clarity, etc. Such subjective aspects are better handled using cognitive information. One such source of cognitive information is gaze behaviour. In this paper, we show that gaze behaviour does indeed help in effectively predicting the rating of text quality. To do this, we first model text quality as a function of three properties - organization, coherence and cohesion. Then, we demonstrate how capturing gaze behaviour helps in predicting each of these properties, and hence the overall quality, by reporting improvements obtained by adding gaze features to traditional textual features for score prediction. We also hypothesize that if a reader has fully understood the text, the corresponding gaze behaviour would give a better indication of the assigned rating, as opposed to partial understanding. Our experiments validate this hypothesis by showing greater agreement between the given rating and the predicted rating when the reader has a full understanding of the text.

==> Instructions.tex <==
\section{Credits}

This document has been adapted from the instructions for earlier ACL and NAACL proceedings, including those for ACL 2017 by Dan Gildea and Min-Yen Kan, NAACL 2017 by Margaret Mitchell, ACL 2012 by Maggie Li and Michael White, those from ACL 2010 by Jing-Shing Chang and Philipp Koehn, those for ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, those for ACL 2005 by Hwee Tou Ng and Kemal Oflazer, those for ACL 2002 by Eugene Charniak and Dekang Lin, and earlier ACL and EACL formats. Those versions were written by several people, including John Chen, Henry S. Thompson and Donald Walker. Additional elements were taken from the formatting instructions of the {\em International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.

\section{Introduction}

The following instructions are directed to authors of papers submitted to ACL 2018 or accepted for publication in its proceedings. All authors are required to adhere to these specifications. Authors are required to provide a Portable Document Format (PDF) version of their papers. \textbf{The proceedings are designed for printing on A4 paper.}

\section{General Instructions}

Manuscripts must be in two-column format.  Exceptions to the two-column format include the title, authors' names and complete addresses, which must be centered at the top of the first page, and any full-width figures or tables (see the guidelines in Subsection~\ref{ssec:first}). \textbf{Type single-spaced.}  Start all pages directly under the top margin. See the guidelines later regarding formatting the first page.  The manuscript should be printed single-sided and its length should not exceed the maximum page limit described in Section~\ref{sec:length}. Pages are numbered for  initial submission. However, \textbf{do not number the pages in the camera-ready version}.

By uncommenting {\verb|\aclfinalcopy|} at the top of this document, it will compile to produce an example of the camera-ready formatting; by leaving it commented out, the document will be anonymized for initial submission.  When you first create your submission on softconf, please fill in your submitted paper ID where {\verb|***|} appears in the {\verb|\def\aclpaperid{***}|} definition at the top.

The review process is double-blind, so do not include any author information (names, addresses) when submitting a paper for review. However, you should maintain space for names and addresses so that they will fit in the final (accepted) version.  The ACL 2018 \LaTeX\ style will create a titlebox space of 6.35 cm for you when {\verb|\aclfinalcopy|} is commented out.  

\subsection{The Ruler}
The ACL 2018 style defines a printed ruler which should be present in the version submitted for review.  The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.  If you are preparing a document without the provided style files, please arrange for an equivalent ruler to appear on the final output pages.  The presence or absence of the ruler should not change the appearance of any other content on the page.  The camera ready copy should not contain a ruler. (\LaTeX\ users may uncomment the {\verb|\aclfinalcopy|} command in the document preamble.)  

\textbf{Reviewers}: note that the ruler measurements do not align well with lines in the paper -- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly. In most cases one would expect that the approximate location will be adequate, although you can also use fractional references ({\em e.g.}, the first paragraph on this page ends at mark $117.5$).

\subsection{Electronically-available resources}

ACL provides this description in \LaTeX2e{} ({\small\tt acl2018.tex}) and PDF format ({\small\tt acl2018.pdf}), along with the \LaTeX2e{} style file used to format it ({\small\tt acl2018.sty}) and an ACL bibliography style ({\small\tt acl\_natbib.bst}) and example bibliography ({\small\tt acl2018.bib}). These files are all available at \url{http://acl2018.org/downloads/acl18-latex.zip}.

A Microsoft Word template file ({\small\tt acl18-word.docx}) and example submission pdf ({\small\tt acl18-word.pdf}) is available at \url{http://acl2018.org/downloads/acl18-word.zip}. We strongly recommend the use of these style files, which have been
appropriately tailored for the ACL 2018 proceedings.

\subsection{Format of Electronic Manuscript}
\label{sect:pdf}

For the production of the electronic manuscript you must use Adobe's Portable Document Format (PDF). PDF files are usually produced from \LaTeX\ using the \textit{pdflatex} command. If your version of \LaTeX\ produces Postscript files, you can convert these into PDF using \textit{ps2pdf} or \textit{dvipdf}. On Windows, you can also use Adobe Distiller to generate PDF.

Please make sure that your PDF file includes all the necessary fonts (especially tree diagrams, symbols, and fonts with Asian characters). When you print or create the PDF file, there is usually an option in your printer setup to include none, all or just non-standard fonts.  Please make sure that you select the option of including ALL the fonts. \textbf{Before sending it, test your PDF by printing it from a computer different from the one where it was created.} Moreover, some word processors may generate very large PDF files, where each page is rendered as an image. Such images may reproduce poorly. In this case, try alternative ways to obtain the PDF. One way on some systems is to install a driver for a postscript printer, send your document to the printer specifying ``Output to a file'', then convert the file to PDF.

It is of utmost importance to specify the \textbf{A4 format} (21 cm x 29.7 cm) when formatting the paper. When working with {\tt dvips}, for instance, one should specify {\tt -t a4}. Or using the command \verb|\special{papersize=210mm,297mm}| in the latex preamble (directly below the \verb|\usepackage| commands). Then using {\tt dvipdf} and/or {\tt pdflatex} which would make it easier for some.

Print-outs of the PDF file on A4 paper should be identical to the hardcopy version. If you cannot meet the above requirements about the production of your electronic submission, please contact the publication chairs as soon as possible.

\subsection{Layout}
\label{ssec:layout}

Format manuscripts two columns to a page, in the manner these instructions are formatted. The exact dimensions for a page on A4 paper are:

\begin{itemize}
\item Left and right margins: 2.5 cm
\item Top margin: 2.5 cm
\item Bottom margin: 2.5 cm
\item Column width: 7.7 cm
\item Column height: 24.7 cm
\item Gap between columns: 0.6 cm
\end{itemize}

\noindent Papers should not be submitted on any other paper size. If you cannot meet the above requirements about the production of your electronic submission, please contact the publication chairs above as soon as possible.

\subsection{Fonts}

For reasons of uniformity, Adobe's \textbf{Times Roman} font should be used. In \LaTeX2e{} this is accomplished by putting

\begin{quote}
\begin{verbatim}
\usepackage{times}
\usepackage{latexsym}
\end{verbatim}
\end{quote}
in the preamble. If Times Roman is unavailable, use \textbf{Computer Modern Roman} (\LaTeX2e{}'s default). Note that the latter is about 10\% less dense than Adobe's Times Roman font.

\begin{table}[t!]
\begin{center}
\begin{tabular}{|l|rl|}
\hline \bf Type of Text & \bf Font Size & \bf Style \\ \hline
paper title & 15 pt & bold \\
author names & 12 pt & bold \\
author affiliation & 12 pt & \\
the word ``Abstract'' & 12 pt & bold \\
section titles & 12 pt & bold \\
subsection titles & 11 pt & bold \\
document text & 11 pt  &\\
captions & 11 pt & \\
abstract text & 11 pt & \\
bibliography & 10 pt & \\
footnotes & 9 pt & \\
\hline
\end{tabular}
\end{center}
\caption{\label{font-table} Font guide. }
\end{table}

\subsection{The First Page}
\label{ssec:first}

Center the title, author name(s), and affiliation(s) across both columns (or, for the initial submission, \textbf{Anonymous ACL submission} for names and affiliations). Do not use footnotes for affiliations. Include the paper ID number assigned during the submission process in the header. Use the two-column format only when you begin the abstract.

\textbf{Title}: Place the title centered at the top of the first page, in a 15-point bold font. (For a complete guide to font sizes and styles, see Table~\ref{font-table}) Long titles should be typed on two lines without a blank line intervening. Approximately, put the title at 2.5 cm from the top of the page, followed by a blank line, then the author name(s), and the affiliation(s) on the following line. Do not use only initials for given names (middle initials are allowed). Do not format surnames in all capitals ({\em e.g.}, use ``Mitchell'' not ``MITCHELL'').  Do not format title and section headings in all capitals as well except for proper names (such as ``BLEU'') that are conventionally in all capitals.  The affiliation should contain the author's complete address, and if possible, an electronic mail address. Start the body of the first page 7.5 cm from the top of the page.

The title, author names and addresses should be completely identical to those entered to the electronic paper submission website in order to maintain the consistency of author information among all publications of the conference. If they are different, the publication chairs may resolve the difference without consulting with you; so it is in your own interest to double-check that the information is consistent.

\textbf{Abstract}: Type the abstract at the beginning of the first column. The width of the abstract text should be smaller than the width of the columns for the text in the body of the paper by about 0.6 cm on each side. Center the word \textbf{Abstract} above the body of the abstract using the font size and style shown in Table~\ref{font-table}. The abstract should be a concise summary of the general thesis and conclusions of the paper. It should be no longer than 200 words. The font size of the abstract text should be as shown in Table~\ref{font-table}. 

\textbf{Text}: Begin typing the main body of the text immediately after the abstract, observing the two-column format as shown in the present document. Do not include page numbers in the final version.

\textbf{Indent}: Indent when starting a new paragraph, about 0.4 cm.

\begin{table}
\centering
\small
\begin{tabular}{cc}
\begin{tabular}{|l|l|}
\hline
\textbf{Command} & \textbf{Output}\\\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular} & 
\begin{tabular}{|l|l|}
\hline
\textbf{Command} & \textbf{ Output}\\\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\\hline
\end{tabular}
\end{tabular}
\caption{Example commands for accented characters, to be used in, {\em e.g.}, \BibTeX\ names.}\label{tab:accents}
\end{table}

\subsection{Sections}

\textbf{Headings}: Type and label section and subsection headings in the style shown on the present document.  Use numbered sections (Arabic numerals) in order to facilitate cross references. Number subsections with the section number and the subsection number separated by a dot, in Arabic numerals. Do not number subsubsections ({\em i.e.}, use \verb|\subsubsection*| instead of \verb|\subsubsection|).

\begin{table*}
\centering
\begin{tabular}{lll}
  output & natbib & previous ACL style files\\
  \hline
  \citep{Gusfield:97} & \verb|\citep| & \verb|\cite| \\
  \citet{Gusfield:97} & \verb|\citet| & \verb|\newcite| \\
  \citeyearpar{Gusfield:97} & \verb|\citeyearpar| & \verb|\shortcite| \\
\end{tabular}
\caption{Citation commands supported by the style file. The citation style is based on the natbib package and supports all natbib citation commands. It also supports commands defined in previous ACL style files for compatibility.}
\end{table*}

\textbf{Citations}: Citations within the text appear in parentheses as~\cite{Gusfield:97} or, if the author's name appears in the text itself, as Gusfield~\shortcite{Gusfield:97}. Using the provided \LaTeX\ style, the former is accomplished using {\verb|\cite|} and the latter with {\verb|\shortcite|} or {\verb|\newcite|}. Collapse multiple citations as in~\cite{Gusfield:97,Aho:72}; this is accomplished with the provided style using commas within the {\verb|\cite|} command, {\em e.g.}, {\verb|\cite{Gusfield:97,Aho:72}|}. Append lowercase letters to the year in cases of ambiguities. Treat double authors as in~\cite{Aho:72}, but write as in~\cite{Chandra:81} when more than two authors are involved. 

Also refrain from using full citations as sentence constituents. We suggest that instead of
\begin{quote}
  ``\cite{Gusfield:97} showed that ...''
\end{quote}
you use
\begin{quote}
``Gusfield \shortcite{Gusfield:97} showed that ...''
\end{quote}

If you are using the provided \LaTeX{} and Bib\TeX{} style files, you can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations.

You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author year'' citations (which is useful for using citations within parentheses, as in \citealp{Gusfield:97}).

If the Bib\TeX{} file contains DOI fields, the paper title in the references section will appear as a hyperlink to the DOI, using the hyperref \LaTeX{} package. To disable the hyperref package, load the style file with the \verb|nohyperref| option: \verb|\usepackage[nohyperref]{acl2018}|.

\textbf{Compilation Issues}: Some of you might encounter the following error during compilation: 

``{\em \verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.}''

This happens when \verb|pdflatex| is used and a citation splits across a page boundary. To fix this, disable the \verb|hyperref| package (see above), recompile and see the problematic citation. Next rewrite that sentence containing the citation. (See, {\em e.g.}, {\small\tt http://tug.org/errors.html})

\textbf{Digital Object Identifiers}:  As part of our work to make ACL materials more widely used and cited outside of our discipline, ACL has registered as a CrossRef member, as a registrant of Digital Object Identifiers (DOIs), the standard for registering permanent URNs for referencing scholarly materials. We are requiring all camera-ready references to contain the appropriate DOIs (or as a second resort, the hyperlinked ACL Anthology Identifier) to all cited works.  Thus, please ensure that you use Bib\TeX\ records that contain DOI or URLs for any of the ACL materials that you reference. Appropriate records should be found for most materials in the current ACL Anthology at \url{http://aclanthology.info/}.

As examples, we cite \cite{P16-1001} to show you how papers with a DOI will appear in the bibliography.  We cite \cite{C14-1001} to show how papers without a DOI but with an ACL Anthology Identifier will appear in the bibliography.  

As reviewing will be double-blind, the submitted version of the papers should not include the authors' names and affiliations. Furthermore, self-references that reveal the author's identity, {\em e.g.},
\begin{quote}
``We previously showed \cite{Gusfield:97} ...''  
\end{quote}
should be avoided. Instead, use citations such as 
\begin{quote}
``\citeauthor{Gusfield:97} \shortcite{Gusfield:97} previously showed ... ''
\end{quote}

\textbf{Please do not use anonymous citations} and do not include acknowledgments when submitting your papers. Papers that do not conform to these requirements may be rejected without review.

\textbf{References}: Gather the full set of references together under the heading \textbf{References}; place the section before any Appendices, unless they contain references. Arrange the references alphabetically by first author, rather than by order of occurrence in the text. Provide as complete a citation as possible, using a consistent format, such as the one for {\em Computational Linguistics\/} or the one in the {\em Publication Manual of the American Psychological Association\/}~\cite{APA:83}.  Use of full names for authors rather than initials is preferred. A list of abbreviations for common computer science journals can be found in the ACM {\em Computing Reviews\/}~\cite{ACM:83}.

The \LaTeX{} and Bib\TeX{} style files provided roughly fit the American Psychological Association format, allowing regular citations, short citations and multiple citations as described above.

\textbf{Appendices}: Appendices, if any, directly follow the text and the references (but see above).  Letter them in sequence and provide an informative title: \textbf{Appendix A. Title of Appendix}.

\subsection{Footnotes}

\textbf{Footnotes}: Put footnotes at the bottom of the page and use the footnote font size shown in Table~\ref{font-table}. They may be numbered or referred to by asterisks or other symbols.\footnote{This is how a footnote should appear.} Footnotes should be separated from the text by a line.\footnote{Note the line separating the footnotes from the text.}

\subsection{Figures and Tables}

\textbf{Placement}: Place figures and tables in the paper near where they are first discussed, as close as possible to the top of their respective column.

\textbf{Captions}: Provide a caption for every illustration; number each one sequentially in the form:  ``Figure 1: Caption of the Figure.'' ``Table 1: Caption of the Table.''  Type the captions of the figures and tables below the body, using the caption font size shown in Table~\ref{font-table}.

\subsection{Equation}
\label{ssec:eqn}

An example equation is shown below:
\begin{equation}
A=\pi r^2
\end{equation}

The numbering (if any) and alignment of the equations will be done automatically (using \verb|align| or \verb|equation|).

\subsection{Accessibility}
\label{ssec:accessibility}

In an effort to accommodate the color-blind (as well as those printing to paper), grayscale readability for all accepted papers will be encouraged.  Color is not forbidden, but authors should ensure that tables and figures do not rely solely on color to convey critical distinctions. A simple criterion: All curves and points in your figures should be clearly distinguishable without color.

\section{Translation of non-English Terms}

It is also advised to supplement non-English characters and terms with appropriate transliterations and/or translations since not all readers understand all such characters and terms. Inline transliteration or translation can be represented in the order of: original-form transliteration ``translation''.

\section{Length of Submission}
\label{sec:length}

The ACL 2018 main conference accepts submissions of long papers and short papers. Long papers may consist of up to eight (8) pages of content plus unlimited pages for references. Upon acceptance, final versions of long papers will be given one additional page -- up to nine (9) pages of content plus unlimited pages for references -- so that reviewers' comments can be taken into account. Short papers may consist of up to four (4) pages of content, plus unlimited pages for references. Upon acceptance, short papers will be given five (5) pages in the proceedings and unlimited pages for references. 

For both long and short papers, all illustrations and tables that are part of the main text must be accommodated within these page limits, observing the formatting instructions given in the present document. Supplementary material in the form of appendices does not count towards the page limit.

However, note that supplementary material should be supplementary (rather than central) to the paper, and that reviewers may ignore supplementary material when reviewing the paper (see Appendix \ref{sec:supplemental}). Papers that do not conform to the specified length and formatting requirements are subject to be rejected without review.

Workshop chairs may have different rules for allowed length and whether supplemental material is welcome. As always, the respective call for papers is the authoritative source.

\section*{Acknowledgments}

The acknowledgments should go immediately before the references.  Do not number the acknowledgments section ({\em i.e.}, use \verb|\section*| instead of \verb|\section|). Do not include this section when submitting your paper for review.

